Multi-Scale Neighborhood Occupancy Masked Autoencoder for Self-Supervised Learning in LiDAR Point Clouds

Masked autoencoders (MAE) have shown tremendous potential for self-supervised learning (SSL) in vision and beyond. However, point clouds from LiDARs used in automated driving are particularly challenging for MAEs since large areas of the 3D volume are empty. Consequently, existing work suffers from leaking occupancy information into the decoder and has significant computational complexity, thereby limiting the SSL pre-training to only 2D bird's eye view encoders in practice. In this work, we propose the novel neighborhood occupancy MAE (NOMAE) that overcomes the aforementioned challenges by employing masked occupancy reconstruction only in the neighborhood of non-masked voxels. We incorporate voxel masking and occupancy reconstruction at multiple scales with our proposed hierarchical mask generation technique to capture features of objects of different sizes in the point cloud. NOMAEs are extremely flexible and can be directly employed for SSL in existing 3D architectures. We perform extensive evaluations on the nuScenes and Waymo Open datasets for the downstream perception tasks of semantic segmentation and 3D object detection, comparing with both discriminative and generative SSL methods. The results demonstrate that NOMAE sets the new state-of-the-art on multiple benchmarks for multiple point cloud perception tasks.

==> figure_latex/NeighOcc.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{\linewidth}
    \centering

    % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=0.7\textwidth]{figure/NeighOcc}
  \end{subfigure}
  \caption{exmaple for niehg occ}
  \hfill
  % \caption{\textbf{noMAE} is the first multi-scale SSL paradigm for automotive point clouds. Using our three main components of: efficient \textbf{n}eighboring \textbf{o}ccupancy \textbf{MAE}, mutli-scale pretexts and a novel heirarechal mask generation, noMAE learns a strong hierarchal representation. Finetuning the pretrained models leads to SOTA downstream performance on three different benchmarks. As can be seen in the figure noMAE improves Nuscenes semseg by 1.4 mIoU, Waymo semseg by 1.0 mIou and Nuscenes objdet by \TODO{...} without the use of extra data.}
  \label{fig:NeighOcc}
\end{figure*}

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,allcolors=cvprblue]{hyperref}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% \setcounter{figure}{9}
% \setcounter{table}{13}
% \setcounter{equation}{5}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter value to the
% % number of references you have in the main paper (here, 100).
% \makeatletter
% \apptocmd{\thebibliography}{\global\c@NAT@ctr 42\relax}{}{}
% \makeatother

% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{1815} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2025}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{Multi-Scale Neighborhood Occupancy Masked Autoencoder for Self-Supervised Learning in LiDAR Point Clouds}  % **** Enter the paper title here

% \maketitle
% \thispagestyle{empty}
% \appendix

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
% We sincerely thank the reviewers for their valuable comments and constructive feedback, and appreciate the comments that NOMAE
% "\textit{is well organized and presented}" and achieves "state-of-the-art performance"{\color{red}(TH88)}. "\textit{the motivation is clear}", proposes "\textit{several novel designs to address the problems}" and "\textit{proposes reconstructing occupancy only in the neighborhood of non-masked voxels}", "\textit{clearly explains the technical details}", "\textit{The proposed method is novel with great performance}", and "\textit{the field can learn knowledge from this paper}"{\color{green}(LNUj)}. "\textit{addresses challenges in masked autoencoders for sparse 3D data}","\textit{A good trade-off}", \textit{experiments are extensive and thorough}" and "\textit{scalability with finer voxel resolutions}"{\color{blue}(bhU8)}. 
% %Below we respond to the main points raised and will incorporate the suggestions in the final version.
% We hope that below clarifications and experiments, thanks to the reviewers comments, will increase the papers value to make it suitable for CVPR. 
% %We are sure that the additional insights from addressing reviewers main points increase our papers value. 

% \noindent\textbf{{\color{red}(TH88)}"\textit{The claimed novelty, i.e., multi-scale and hierarchical masking scheme may not be qualified for CVPR}":}
% In addition to the mentioned novelties by the reviewer, we claim Neighborhood Occupancy MAE as a novelty contribution. 
% NOMAE is the first \textsl{localized reconstruction} self-supervised learning framework. 
% This efficiently solves the positional information leakage problem of standard MAE on point clouds, while being better suited for large sparse point clouds compared to full-scene reconstruction in earlier works [23,36].
% NOMAE is more effective for representation learning on large scenes,
% adding $7.7$~mIoU over existing SSL methods in Tab.~4. 
% %We show in Tab. 4 that reconstructing only the neighborhood adds 7.7 mIoU when probing the learned representation for Semseg, compared to full scene reconstruction. 
% Single-scale NOMAE needs only a fraction of computational capacity for pretraining compared to earlier works [23,36], enabling supervision at finer scales and at multiple feature levels. %We will change "sparse" to "localized reconstruction" in line 80 to make the contribution clearer.
% We will reformulate the corresponding parts in the paper to make this contribution clearer. 

% \noindent\textbf{{\color{red}(TH88)}"\textit{As said in sec 3.3, muli-scale idea has been used in Geo-MAE, although in a different way}":}
% MSP in NOMAE assigns different reconstruction target sets to different layers of different granularity, promoting feature diversity between layers. In contrast, GEO-MAE reconstructs a voxel sub-occupancy at multiple scales, but only from a single feature layer.
% This does not promote feature diversity and makes the layer a bottleneck. 
% Results in Tab.~3 quantify the performance gain of NOMAE over GEO-MAE. 
% Our ablation in the table below adds further evidence by varying only the multi-scale target (GEO-MAE vs our MSP).
% The gain from MSP is $\sim3\times$ GeoMAE's MS on Nuscenes Semseg val set. 
% We will add this experiment to the ablations.
% \begin{table}[h]
%     \centering
%     % \addtolength{\tabcolsep}{-0.5em}
%     \footnotesize
%     \vspace{-2.5em}
%     \begin{tabular}{ccc}
%         SS $2^s=8$ NOMAE& +GEO-MAE's MS& +our MSP\\
%         \midrule
%         68.3 & 69.7 & \textbf{72.6}\\
%     \end{tabular}
%     \vspace{-2.0em}
%     \label{tab:convergence_semseg}
% \end{table}

% \noindent\textbf{{\color{red}(TH88)}"\textit{Hierarchical masking seems quite straightforward}":}
% We agree with the reviewer, yet the simplicity of HMG adds to its elegance. 
% HMG ensures consistent masking ratios across scales, balancing coarse and fine feature learning. 
% The effectiveness of HMG is supported by the results in Tab.~4, which compare it to previously proposed masking schemes.

% \noindent\textbf{{\color{red}(TH88)}"\textit{Tight coupling with PTv3}",{\color{green}(LNUj)}"\textit{demonstrate the generalizability of NOMAE}":}
% %We thank them for directing us to test the generalization of NOMAE to other architectures. 
% The paper used PTv3 since it is the strongest baseline model on many datasets. 
% Clearly, we agree with the reviewers that a good SSL method should be applicable to a variety of models, including CNNs and transformers. 
% We thank the reviewers for highlighting this important issue. 

% Below, we present results on Nuscenes Semseg val set for SPUnet [9], OACNNs \href{https://openaccess.thecvf.com/content/CVPR2024/papers/Peng_OA-CNNs_Omni-Adaptive_Sparse_CNNs_for_3D_Semantic_Segmentation_CVPR_2024_paper.pdf}{[43]}, and Octformer \href{https://ojs.aaai.org/index.php/AAAI/article/view/25121/24893}{[44]}.
% %We use the same settings as in Sec. 4.3 and Sec. 6 except for the learning rate. 
% NOMAE improves the mIoU by 1.8 points on average, even without optimization of hyperparameters, which we could not perform given the limited rebuttal time period. We hypothesize, NOMAE's generalization arises from the feature diversity promoted by MSP.
% We will add the table to the ablations.
% % To the best of our knoweldge, these concepts(i.e. localized reconstruction, MS-SSL at multiple feature levels, Hierarchal Masking) were never introduced in earlier works, and our extensive experiments demonstrate the benefit of each of those contributions. 
% \begin{table}[h]
%     \centering
%     \footnotesize
%     \vspace{-1.em}
%     \addtolength{\tabcolsep}{-0.5em}
%     \begin{tabular}{lcccccc}
%     \toprule
%     \textbf{Model} & \multicolumn{2}{c}{Scratch(paper)} & \multicolumn{2}{c}{Scratch(ours)} & \multicolumn{2}{c}{+ NOMAE}\\
%     & \textbf{mIoU} & \textbf{mACC} & \textbf{mIoU} & \textbf{mACC}& \textbf{mIoU} & \textbf{mACC} \\
%     \midrule
%       SPUnet\,[9] &73.3&-&78.6&83.9&80.1&86.2\\ % number of original paper
%       OACNNs\,\href{https://openaccess.thecvf.com/content/CVPR2024/papers/Peng_OA-CNNs_Omni-Adaptive_Sparse_CNNs_for_3D_Semantic_Segmentation_CVPR_2024_paper.pdf}{[43]}   &78.9&-&78.8&85.8&80.9&86.4\\ 
%       Octformer\,\href{https://ojs.aaai.org/index.php/AAAI/article/view/25121/24893}{[44]} &-&-&78.4&86.9&80.2&\textbf{88.2}\\ 
%       PTv3[31] &80.4&-&80.4&87.3&\textbf{81.8}&87.7\\ 
%     \bottomrule
%     \end{tabular}
%     \vspace{-1.7em}
% \end{table}

% \noindent\textbf{{\color{blue}(bhU8)}{Results at convergence}:} 
% The results of our baselines in Tab.~1 are taken from the original papers, thus after convergence. 
% Below, we provide additional results for longer training schedules of $50$, $100$ and $200$ epochs from scratch. 
% Results show no significant improvement through longer training, confirming that NOMAE improves sample efficiency. 
% We will add the experiment to the paper. 

% \begin{table}[h]
%     \centering
%     \footnotesize
%     \vspace{-1.0em}
%     \begin{tabular}{cccccc}
%         Sup,50 ep~[31]& Sup, 100ep& Sup, 200ep & NOMAE+50ep\\
%         \midrule
%         80.4 & 80.7 & 80.6& \textbf{81.8}\\
%     \end{tabular}
%     \vspace{-1.5em}
% \end{table}

% For object detection, results after convergence are showing a performance gain through NOMAE, even with only $40$ epochs of training:
% \begin{table}[h]
%     \centering
%     \footnotesize
%     \addtolength{\tabcolsep}{-0.25em}
%     \vspace{-1.5em}
%     \begin{tabular}{l|ccc|cc}
%         &\multicolumn{3}{c}{Scratch}&\multicolumn{2}{c}{NOMAE}\\
%         &20ep~[37]&300ep&400ep&20ep&40ep\\

%         \midrule
%         NDS/mAP&46.7/39.0& 64.1/56.8& 64.2/56.7 & 60.9/54.5 & \textbf{64.9}/\textbf{58.9}\\

%     \end{tabular}
%     \vspace{-1.5em}
%     \label{tab:convergence_objdet}
% \end{table}

% \noindent\textbf{{\color{blue}(bhU8)}{Object sample augmentation}:} 
% We agree with the reviewer, object sample's database should only use the $20\%$ labeled data.
% For this reason, \textsl{we did not use} object sample at all. 
% Additionally, This makes our evaluation consistent with SSL literature [37]. 
% %
% %We don't use Object sample augmentation during finetuning or pretraining. 
% %We refereed to it as copy paste augmentation in the caption of Tab. 2. 
% %We choose to train only for 20 epochs to directly compare with other SSL methods. 
% %We didn't use Object sample for the same reason. 
% %As reviewer noted, this is not enough for convergence. 
% %Results at convergence using for the same setup are as follows,
% Below we show results using $100\%$ labeled data, CBGS (1 epoch equals 5 epochs without CBGS), \textsl{with object sample augmentation}:
% % \begin{table}[h]
% %     \centering
% %     \footnotesize
% %     % \caption{Objdet mAP and NDS for 100\% labeled data, with CBGS, and object sample}
% %     \addtolength{\tabcolsep}{-0.5em}
% %     \vspace{-0.5em}
% %     \begin{tabular}{lcccc}
% %         &backbone&epochs&NDS& mAP\\
% %         \midrule
% %         UVTR~[20] & SpConv& 20 &67.7 &60.9\\
% %         +NOMAE & SpConv& 5& \textbf{\color{red}todo}&\textbf{\color{red}todo}\\

% %         UVTR & PTv3& 20& 69.3&64.1 \\
% %         +NOMAE & PTv3& 5& \textbf{71.2}&\textbf{67.0} \\
% %     \end{tabular}
% %     \vspace{-1.0em}
% %     \label{tab:convergence_objdet}
% % \end{table}

% %\begin{table}[h]
% %    \centering
% %    \footnotesize
%     % \caption{Objdet mAP and NDS for 20\% labeled data, no CBGS, and no object sample}
%     % \addtolength{\tabcolsep}{-0.25em}
% %    \vspace{-1.5em}
% %    \begin{tabular}{l|cc|cc}
% %        &\multicolumn{2}{c}{Scratch 20ep}&\multicolumn{2}{c}{NOMAE+5ep}\\
% %        backbone&SpConv~[37]&PTv3&SpConv&PTv3\\
% %        
% %        \midrule
% %        NDS/mAP&67.7/60.9& 69.3/64.1& {\color{red}todo} & \textbf{71.2}/\textbf{67.0} \\
% %    \end{tabular}
% %    \vspace{-1.0em}
% %\end{table}

% \begin{table}[h]
%     \centering
%     \footnotesize
%     % \caption{Objdet mAP and NDS for 20\% labeled data, no CBGS, and no object sample}
%     % \addtolength{\tabcolsep}{-0.25em}
%     \vspace{-1.em}
%     \begin{tabular}{l|c|c}
%         NDS/mAP&{Scratch 20ep}&{NOMAE +5ep}\\
        
%         \midrule
%         PTv3&69.3/64.1& \textbf{71.2}/\textbf{67.0} \\
%         SPConv~[37]&67.7/60.9& 70.4/65.3 \\
%     \end{tabular}
%     \vspace{-1.0em}
% \end{table}

% %The results shows that in addition to greatly improving convergence speed, NOMAE improves sample efficiency. We will state it clearly in our results and implementation details.

% % After receiving paper reviews, authors may optionally submit a rebuttal to address the reviewers' comments, which will be limited to a {\bf one page} PDF file.
% % Please follow the steps and style guidelines outlined below for submitting your author response.

% % The author rebuttal is optional and, following similar guidelines to previous conferences, is meant to provide you with an opportunity to rebut factual errors or to supply additional information requested by the reviewers.
% % It is NOT intended to add new contributions (theorems, algorithms, experiments) that were absent in the original submission and NOT specifically requested by the reviewers.
% % You may optionally add a figure, graph, or proof to your rebuttal to better illustrate your answer to the reviewers' comments.

% % Per a passed 2018 PAMI-TC motion, reviewers should refrain from requesting significant additional experiments for the rebuttal or penalize for lack of additional experiments.
% % Authors should refrain from including new experimental results in the rebuttal, especially when not specifically requested to do so by the reviewers.
% % Authors may include figures with illustrations or comparison tables of results reported in the submission/supplemental material or in other papers.

% % Just like the original submission, the rebuttal must maintain anonymity and cannot include external links that reveal the author identity or circumvent the length restriction.
% % The rebuttal must comply with this template (the use of sections is not required, though it is recommended to structure the rebuttal for ease of reading).

% % %-------------------------------------------------------------------------

% % \subsection{Response length}
% % Author responses must be no longer than 1 page in length including any references and figures.
% % Overlength responses will simply not be reviewed.
% % This includes responses where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% % Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.

% % %------------------------------------------------------------------------
% % \section{Formatting your Response}

% % {\bf Make sure to update the paper title and paper ID in the appropriate place in the tex file.}

% % All text must be in a two-column format.
% % The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% % Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% % The top margin should begin 1 inch (2.54 cm) from the top edge of the page.
% % The bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% % for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the page.

% % Please number any displayed equations.
% % It is important for readers to be able to refer to any particular equation.

% % Wherever Times is specified, Times Roman may also be used.
% % Main text should be in 10-point Times, single-spaced.
% % Section headings should be in 10 or 12 point Times.
% % All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% % Figure and table captions should be 9-point Roman type as in \cref{fig:onecol}.


% % List and number all bibliographical references in 9-point Times, single-spaced,
% % at the end of your response.
% % When referenced in the text, enclose the citation number in square brackets, for example~\cite{Alpher05}.
% % Where appropriate, include the name(s) of editors of referenced books.

% % \begin{figure}[t]
% %   \centering
% %   \fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
% %   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
% %    \caption{Example of caption.  It is set in Roman so that mathematics
% %    (always set in Roman: $B \sin A = A \sin B$) may be included without an
% %    ugly clash.}
% %    \label{fig:onecol}
% % \end{figure}

% % To avoid ambiguities, it is best if the numbering for equations, figures, tables, and references in the author response does not overlap with that in the main paper (the reviewer may wonder if you talk about \cref{fig:onecol} in the author response or in the paper).
% % See \LaTeX\ template for a workaround.

% % %-------------------------------------------------------------------------
% % \subsection{Illustrations, graphs, and photographs}

% % All graphics should be centered.
% % Please ensure that any point you wish to make is resolvable in a printed copy of the response.
% % Resize fonts in figures to match the font in the body text, and choose line widths which render effectively in print.
% % Readers (and reviewers), even of an electronic copy, may choose to print your response in order to read it.
% % You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% % When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the  figure width as a multiple of the line width as in the example below
% % {\small\begin{verbatim}
% %    \usepackage{graphicx} ...
% %    \includegraphics[width=0.8\linewidth]
% %                    {myfile.pdf}
% % \end{verbatim}
% % }


% %%%%%%%%% REFERENCES
% % {
% %     \small
% %     \bibliographystyle{ieeenat_fullname}
% %     \bibliography{main}
% % }

% \end{document}


==> table/k_size.tex <==
% this table should just be a single row where every col is a different reconstructoin size. I only have NonLP numbers on  nuscenes
\begin{tabular}{l c c c c c}\toprule
  &&&&&\\
\midrule
  &&&&&\\
  &&&&&\\
 &&&&&\\
 &&&&&\\
 &&&&&\\
 &&&&&\\
\bottomrule
\end{tabular}



==> table/rebuttal/other_architectures.tex <==
% This table would be semseg only on nuscenes. we can report any method that reported semseg. and also we report the 4 different runs I have for the 2 reimplemented methods (occmae  and geomae). I want to report LLRD and NonLP
%
% Incremental results
%
\addtolength{\tabcolsep}{-0.5em}
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \multicolumn{2}{c}{Scratch(paper)} & \multicolumn{2}{c}{Scratch(ours)} & \multicolumn{2}{c}{+ NOMAE}\\
& \textbf{mIoU} & \textbf{mACC} & \textbf{mIoU} & \textbf{mACC}& \textbf{mIoU} & \textbf{mACC} \\
% \midrule
%   GEO-MAE\,\citep{tian2023geomae}$^{*}$ &78.6&-&-\\ % number of original paper
%   GEO-MAE + PTv3$^{*}$ &78.9&84.7&94.4\\
%   Occupancy-MAE\,\citep{min2022OccupancyMAESP}$^{*}$ &72.9&-&-\\  % number of original paper
%   Occupancy-MAE + PTv3$^{*}$ &80.0&86.1&94.6\\% number of your re-implementation with PTv3
%   UniPAD\,~\citep{Yang2023UniPADAU}&79.4&-&-\\
% %  PTv3 &&&\\ % number of original paper
\midrule
  SPUnet\,\citep{tian2023geomae} &73.3&-&78.6&83.9&80.1&86.2\\ % number of original paper
  OACNNs\,\citep{Peng2024OACNNsOS}   &78.9&-&78.8&85.8&80.9&86.4\\ % number of your re-implementation with PTv3
  Octformer\,\citep{Wang2023OctFormerOT} &-&-&77.2&86.2&\color{red}{todo} &\color{red}{todo}\\ % number of your re-implementation with PTv3
\bottomrule
\end{tabular}

